Fourier Domain Synthesis Imaging Using A Wirelessly Coordinated Distributed Antenna Array

In this work we present an experimental demonstration of one-dimensional Fourier-domain imaging using a fully-digital wirelessly coordinated coherent distributed antenna array (CDA) receiver. The nodes consist of two software-defined radios (SDRs) operating with independent system clocks performing wireless time, frequency, and phase coordination without a shared reference such as the global navigation satellite system (GNSS). Two spatially separated noise sources transmit independent noise waveforms with a bandwidth of 25 MHz and a carrier frequency of 915 MHz. Two sources were positioned at angles of $-6.28{\deg}$ and $12.95{\deg}$ off broadside and imaging was performed. The two sources are clearly resolved to within $3{\deg}$ of their expected locations in both the individual and combined source measurements and demonstrating the Fourier-domain image reconstruction principle using a fully-digitally coordinated distributed antenna array.

==> ieee_submission_notice.tex <==
\makeatletter
\def\ps@IEEEtitlepagestyle{%
  \def\@oddfoot{\mycopyrightnotice}%
  \def\@oddhead{\hbox{}\@IEEEheaderstyle\leftmark\hfil\thepage}\relax
  \def\@evenhead{\@IEEEheaderstyle\thepage\hfil\leftmark\hbox{}}\relax
  \def\@evenfoot{}%
}
\def\mycopyrightnotice{%
  \begin{minipage}{\textwidth}
  \centering \scriptsize
  This work has been submitted to the IEEE for possible publication. Copyright may be transferred without notice, after which this version may no longer be accessible.
  \end{minipage}
}
\makeatother
